URDFormer: A Pipeline for Constructing Articulated Simulation Environments from Real-World Images

Constructing simulation scenes that are both visually and physically realistic is a problem of practical interest in domains ranging from robotics to computer vision. This problem has become even more relevant as researchers wielding large data-hungry learning methods seek new sources of training data for physical decision-making systems. However, building simulation models is often still done by hand. A graphic designer and a simulation engineer work with predefined assets to construct rich scenes with realistic dynamic and kinematic properties. While this may scale to small numbers of scenes, to achieve the generalization properties that are required for data-driven robotic control, we require a pipeline that is able to synthesize large numbers of realistic scenes, complete with 'natural' kinematic and dynamic structures. To attack this problem, we develop models for inferring structure and generating simulation scenes from natural images, allowing for scalable scene generation from web-scale datasets. To train these image-to-simulation models, we show how controllable text-to-image generative models can be used in generating paired training data that allows for modeling of the inverse problem, mapping from realistic images back to complete scene models. We show how this paradigm allows us to build large datasets of scenes in simulation with semantic and physical realism. We present an integrated end-to-end pipeline that generates simulation scenes complete with articulated kinematic and dynamic structures from real-world images and use these for training robotic control policies. We then robustly deploy in the real world for tasks like articulated object manipulation. In doing so, our work provides both a pipeline for large-scale generation of simulation environments and an integrated system for training robust robotic control policies in the resulting environments.

==> script/rebuttal.tex <==
%\begin{titlepage}
 
\twocolumn[ 
\begin{center}
     {\Large URDFormer: A Pipeline for Constructing Articulated Simulation Environments from Real-World Images \par}
    \vspace{0.5cm}
    {\Large Rebuttal: Feedback from Reviewers}
\end{center}

{\centering
    \includegraphics[width=\textwidth]{figures/rebuttal_summary_scenes.png}
    \captionof{figure}{A summary of categories of objects and scenes that we trained \method to predict. We visualize examples of \method predictions (large background image) given corresponding internet images (small overlaid black box). (\textcolor{blue}{Blue}) shows categories of scenes and objects that are new in the rebuttal, while black shows the original categories. We train a single part \method for all object categories and a single global \method for all scene categories.
    %To make it clear, under each object category, we also list out how we divide the object parts.
    Under each object category, we also list the individual articulated parts that it contains.
    See more visualizations for each new category in Section \ref{sec:rebuttal_generalization}.}
    \label{fig:summary_figure}
     \vspace{0.5cm}
}
]
We would like to thank all the reviewers and the area chair for their thoughtful and detailed feedback. We will first reply to the main concerns on scalability, followed by individual responses to each reviewer. All the main changes to the original draft are highlighted in \textcolor{blue}{blue}.
% Several reviewers requested experiments with more diverse objects and scenes and more complex tasks and robots. We have therefore grouped our responses to these issues, and address further reviewer-specific responses below.

\section*{General Response 1: Applicability to wider classes of situations}

%\method is versatile and can be applied to other objects and scenes.
%We
In response to the reviewer comments citing the narrow range of kitchen environments in the original draft, we
extended our training dataset and evaluated \method on 5 new object categories (Study Desk, Microwave, Chair, Laptop and Toilet) and 4 new global scenes (Bedroom, Bathroom, Laundry Room, Study Room), highlighted in blue in Figure \ref{fig:summary_figure}.
%Interestingly, we did not train \method in the Laundry Room and Study Room but found that \method can be applied in these scenarios.  This generalization to unseen categories is likely due to the separate training on the global URDFormer and part URDFormer. 
We found that a \method model trained on the Kitchen, Bathroom and Bedroom environments can be transferred directly to the Laundry Room and Study Room environments, despite not having been trained on these layouts.  This generalization is likely due to the separate training of the global URDFormer and part URDFormer which had seen all the individual object categories.  Please see details and more visualizations in 
Figure \ref{fig:new_dataset} and Figure \ref{fig:new_prediction} under Section \ref{sec:rebuttal_generalization}.
% Please note that \method only predicts kinematics structure and part classes, and does not reconstruct accurate meshes and object properties such as mass. This is our limitation and focus in the future work. -> covered already in the limitation session.

\section*{General Response 2: Complex Tasks and A Different Robot}
The main goal for the \method is to construct articulated simulation content directly from real-world images. This enables faster and cheaper scene generation that also emulate the real-world distribution. The generated scenes can be used to train different robots and tasks. We additionally provide experiments using a Stretch robot. In particular, we generated a dataset based on the URDF prediction of the office desk, and trained a vision-based policy that takes the initial observation, as well as the task embeddings, and predicts an affordance map at each step. These affordance maps are used together with a motion planner to guide the robot at each step. We show \method can be used to train a Stretch robot and complete the task "clean up the table surface", which involves steps of "Open the drawer", "Pick up the object" and "Put the object in the drawer". We provide details on the robot experiments in Section \ref{sec:rebuttal_robot}.

\begin{figure}[H]
  \centering
  \includegraphics[width=0.45\textwidth]{figures/rebuttal_robot_summary.png}
  \caption{We trained a Stretch robot on a multi-step task of "Clean Up the Table Surface" using the training set generated based on URDFormer prediction.}
\end{figure}

%\noindent {\Large Reviewer Specific Responses}
\section*{Reviewer Specific Responses}


Meta Reviewer EEoy
\begin{itemize}
    \item \textit{``...there are some doubts regarding scalability, in terms of applicability to wider classes of situations: Authors are encouraged to extend the application scenarios"}  Thank you for this feedback.  We have provided new experiments with more diverse objects and scenes, as well as more complex tasks with a second robot.  Please see General Response 1 and General Response 2 above.
\end{itemize}

Reviewer CHaG
\begin{itemize}
    \item
    \textit{``Why don't we just use ORB-SLAM, NeRF, or other 3d mapping/reconstruction techniques to get a model of a scene?"}  While many of these techniques have been shown to provide detailed and accurate 3D models of environments, most do not generate articulated structures that can be used to simulate dynamic interactions.  We have added a short clarifying paragraph to the beginning of Section \ref{sec:related_work} (Related Work) to address this confusion.

    \item
    \textit{``There are many techniques involved in the proposed approach. This means there will be a lot of parameters to be optimized and tuned. Then how robust is your proposed learning framework?"}  While it is true that our approach contains multiple separately trained components, each of these has a clearly defined objective that is directly aligned with the downstream task.  For the most part, this allows us to optimize each component separately without worrying about how the hyperparameters of each component affect the entire system.  For example, optimizing the part detector to produce the best local estimates of the door and handle positions will best contribute to the overall system goal of producing the most accurate model of the entire scene.  We have added a brief discussion of this to Section \ref{sec:limitations} (Limitations and Future Work) and Appendix F to clarify these points.

    \item
    \textit{``What is the reason for using the learning components such as ViT, diffusion model, etc.?"}  Each of the models chosen in our system were designed to represent accessible best-practices in current architecture and training design.  While these components may not be the absolute state-of-the-art, they are rather intended to be high-quality models that are easily accessible to other researchers.  A few notes on specific components: A VIT model was chosen for visual feature extraction as they are relatively simple to implement, and do not require substantial tuning.  The generative diffusion components we used are pretrained off-the-shelf models, so we simply chose the most performant publicly available model at the time of submission.  Finally, we use a finetuned Grounding DINO model for detection, as it allowed us to capitalize on the high-quality large-scale initial training run, while still allowing us to customize it to our purposes.  We found that using the Model Soup technique of averaging the weights between our finetuned model and the original pretrained model substantially improved performance, and ensured that the eventual model did not overfit to our finetuning data.
\end{itemize}

Reviewer HiJK
\begin{itemize}
    \item
    \textit{``The main limitation of the work presented in the paper is the relatively narrow scope of the scenes and types of objects in them"}  Please see ``General Response: Diverse Objects and Scenes" above.

    \item
    \textit{``There are also likely relations between textures and inertial properties that are not fully captured/explored in the paper."}  While we are presently not using texture information to infer any kinematic properties of the model, we agree that this could be a valuable line of future work.  We have added a brief discussion of this to Section \ref{sec:limitations} (Limitations and Future Work).

    \item
    \textit{``The only baseline that is not a derivative version of the proposed work turns out not successful at all, making it questionable to include it and leaving the comparisons aspect of the result sections rather scant."} Thank you for this feedback, our goal in including OWL-VIT was to provide a baseline that uses a large-scale open-vocabulary vision and language model in an attempt determine the competitiveness of our learned approach compared with a large-scale model that does not require new training.  As these large pretrained open-vocabulary approaches are rapidly increasing in popularity, we thought this would be a useful comparison.  We have added some additional visualization of the failure modes of this method in Appendix E.

    \item
    \textit{``...referring to what is essentially a very textbook supervised learning problem as the "inverse" problem is a bit confusing."}  This is valuable feedback, thank you for raising the issue.  Our goal in using the forward/inverse framing was to highlight that the inference-time process which turns an image into a URDF prediction is the inverse of the generative process which constructs the training data.  We have added a new paragraph at the beginning of Section \ref{sec:method} which we hope will clarify this.

    \item
    \textit{``It would be appropriate to cite and discuss this work \href{https://arxiv.org/pdf/2203.10488.pdf}{https://arxiv.org/pdf/2203.10488.pdf}..."} Thank you for this reference, we have added it to Section \ref{sec:related_work} (Related Work) under methods which require RGBD data.  The primary difference between our approach and theirs is that we do not require video, and do not require depth information to build articulated models.  This is important when building data using online images, as depth information is rarely available from online sources.  We have added a short sentence clarifying this near the end of the Related Work subsection ``A. Asset Creation for Robot Manipulation."

    \item
    \textit{``approach —leveraging extra space before the em dash} Thank you for noticing this, it has been fixed.
    
    \item
    \textit{``How are the scene and object segmentations mentioned in section I.C obtained?"} We apologize for the confusion, we accidentally used the word ``segmentation" when we meant ``detection."  We do not use pixel-wise segmentation masks, but use 2D bounding boxes generated by the fine-tuned Grounding-DINO model (see Appendix C-A for details) to extract regions of the original image, which are fed to the URDF prediction components.  We have corrected the language in Section \ref{sec:method} to be more clear.
\end{itemize}

Reviewer h1RM
\begin{itemize}
    \item
    \textit{``The proposed approach has so far only been tested in a kitchen environment and the objects examined were mostly cabinets. Further demonstration of the method applied to other scenarios and with different robot types is desired."}  Thank you for this feedback, we have added additional experiments in new environments with a second robot.  Please see ``General Response 1: Applicability To Wider Classes of Situations" and ``General Response 2: Complex Tasks and Robots" above.

    \item
    \textit{``It was explained that the placement of the handles for objects such as a cabinet can be inaccurate and this is resolved through targeted randomization. Could you provide more detail regarding this process? Does this process randomly modify the position and/or shape of the handles in every generation?"} We apologize for the confusion. When training the robot policy with data from the \method predictions, the  handle/knob geometry for the doors and drawers was randomly replaced with alternate handle geometry from PartNet, and randomly shifted slightly in the plane of the door/drawer.  Additionally, the door/drawer geometry was replaced with alternate geometry using PartNet which was scaled to match the appropriate shape.  We have added a clarifying description of this process in Section \ref{sec:two_a}.

    \item
    \textit{``Fig. 2 is missing/skipped in the paper.''} Apologies for this, thank you for pointing it out.  This was a formatting issue causing the labeling to skip from 1 to 3, which has been fixed.

    \item
    \textit{``Several figures (i.e. Fig. 8, 9) and tables (i.e. Table II) are not mentioned in the text. Please refer to the figures in the paper in the appropriate sections."} We apologize for this oversight.  References to the figures and tables have been added throughout the paper.

    \item
    \textit{``For future work, it would be interesting to see how the method handles environments outside of the kitchen scene and whether real robots can train their behavior online upon observing an object it needs to handle."} Thank you for this feedback, we have added some new scenes outside the kitchen and new tasks with a second robot in the ``General Response 1: Applicability to wider classes of situations" and ``General Response 2: Complex Tasks and Robots" sections above.

\end{itemize}

==> script/related_work_old.tex <==
\section{Related Work}
\label{sec:related_work}
% This work is related to a large body of work in inverse-graphics, procedural generation, 3-D reconstruction and data augmentation. We provide some context on these related fields below. 

% \todo{\begin{itemize}
%     \item inverse graphics (shorten or remove)
%     \item data aug w/ generative models
%     \item scene generation (including latest using LLMs)
%     \item sim construction / scene reconstruction
%     \item real to sim to real pipelines (look for ditto in the house ++, shuran songs work) -> already added to Scene Reconstruction
% \end{itemize}}

\textbf{Inverse-Graphics for Scene Reconstruction}:
The field of inverse graphics is interested in inferring the properties of a scene from images (or videos) of the scene of interest. A variety of work focuses on inferring scene properties, e.g., geometry or lighting from single images \citep{battaglia2013simulation} through optimization-\citep{agarwal2011building} or learning-based\citep{park2019deepsdf} approaches.
In a similar vein, a rich body of work ~\citep{3drsurvey} focuses on mesh reconstruction and novel view synthesis using a variety of techniques such as implicit neural fields \citep{mildenhall2021nerf, Park20arxiv_nerfies, Zhang20arxiv_nerf++}, Gaussian splatting \citep{kerbl20233d, luiten2023dynamic}, differentiable rendering \citep{nguyen2018rendernet, kato2020differentiable, liu2018paparazzi} amongst many other techniques. 
% Importantly, the focus of many of these works on inverse graphics has been on geometric reconstruction rather than our focus on scene-level simulation construction complete with kinematic and semantic structure like object relationships and articulation.
Most recently, constructing digital twins has gained popularity in robotics especially to bridge the gap between simulation and reality. Through robotic~\cite{nie2022structure, ma2023sim2real} or human~\cite{hsu2023ditto, jiang2022ditto} interaction data, the articulation and parts of the object are revealed and a simulated model of the object or scene can be constructed.
Others focus on inferring physics parameters, e.g., friction and surface properties \citep{wu2017learning, piloto2022intuitive, kubricht2017intuitive, de2018end}. Training robotic control policies on such reconstructed scenes can allow for zero- or few-shot transfer from simulation to reality.
% In contrast, our work focuses less on exact geometry reconstruction but rather on generating correct scene statistics at the articulation/kinematics/positioning level for entire scenes or complex objects from single RGB images.
\method{} eliminates the need for prior interaction by modeling the reconstruction process directly as an inverse graphics problem. Our method can reconstruct an unseen scene from a single RGB image accurately enough to allow for zero-shot sim2real transfer of robotic control policies.


% As opposed to these methods, the goal is not just a slow and expensive process for a single scene, but a fast generation process that can scale to generate hundreds of scenes with natural statistics. Importantly, this generation process does not require interaction or targeted data collection per domain.
% and instead can operate off of just web-scale image data. 

% TODO: integrate this stuff up. 
% key point - talk about how all of this either uses a known dataset or really focuses on geometry reconstruction. Josh tenenbaum stuff, need to google, ask some vision people. 
% intuitive physics stuff, tejas kulkarni stuff.  Talk about how lots of people try to do either physics inference from real interaction or geometry inference from real data. But less people try to do full scene inference from single RGB images. 
% [3D-Aware Scene Manipulation via Inverse Graphics]
% [tejas kulkarni deep IG]
% [tejas kulkarni IG with CAD]
% [3D-Aware Scene Manipulation via Inverse Graphics]

% Key point: interaction needed. Mention shuran song stuff on dense-phys net and so on - talk about how this needs interaction and depth and so on. More about physics than about diverse, full scene generation with kinematic structure.Jiajun wu stuff on physics interaction

%\textbf{Procedural Scene Generation and Large-Scale Simulation Generation:} Indoor scene synthesis is a long-standing problem in computer vision. For a quick sampling of these works, \citep{chang2014learning, chang2015text} are able to generate certain types of 3D scenes from text descriptions \citep{hu2020graph2plan, nauata2021house, wang21roominoes} learn to generate floor plans, while \citep{ritchie2019fast, keshavarzi2020scenegen, li2019grains, hudson21gansformer} use generative models directly for indoor scene generation. While generating scenes this way can be promising, these methods either fail to achieve the targeted generation of complex scenes with articulation and complex kinematic structure intact or require extremely expensive inference processes to do so. On the other hand, procedural generation techniques have been popular in generating grid-world environments \citep{khalifa2020pcgrl, earle2021learning, dennis2020emergent, linus21procedural} and in generating home environments at scale ~\citep{deitke2022, deitke23phone2proc}. These scenes are diverse and often rich, but are not controllable to particular target scenes or are not able to generate scenes complete with physical properties and articulation. Other techniques such as ~\citep{li21openrooms} are able to generate large datasets of more interactive scenes but require full-depth information and heuristics for dataset generation specific to indoor scenes. \method{} is able to generate realistic, diverse, and controllable scenes while retaining rich kinematic and semantic structure. 

\textbf{Synthetic Scene Generation} Another attempt to narrow the sim2real gap is to generate vast amounts of simulation data without touching the real world. For instance, generating synthetic scenes has been studied by learning generative models of indoor scenes \citep{ritchie2019fast,li2019grains, keshavarzi2020scenegen,hudson21gansformer} and floor plans \citep{hu2020graph2plan, nauata2021house, wang21roominoes}, or using text-to-scene models \citep{chang2014learning, chang2015text}. While generating scenes this way can be promising, these methods either fail to achieve the targeted generation of complex scenes with articulation and complex kinematic structure intact or require extremely expensive inference processes to do so. On the other hand, procedural generation techniques have been popular in generating grid-world environments \citep{khalifa2020pcgrl, earle2021learning, dennis2020emergent, linus21procedural} and in generating home environments at scale ~\citep{deitke2022}. These scenes are diverse and often rich, but are not controllable to particular target scenes or are not able to generate scenes complete with physical properties and articulation. Other techniques such as ~\citep{li21openrooms, deitke23phone2proc} are able to generate large datasets of more interactive scenes but require interactive scanning with either a phone or other hardware for dataset generation specific to indoor scenes. \todo{<- sentence too dense and ambiguous -> clarify difference to URDFormer}
\method{} is able to generate realistic, diverse, and controllable scenes while retaining rich kinematic and semantic structure from internet images alone.


\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/overview_bigfont.pdf}
        \caption{The URDFormer is trained on a large paired dataset of simulation assets and realistic renderings (forward). During inference, this process is inverted and it predicts the URDF from a real image (inverse). \todo{specific what ''supervision'' means -> MSE?}}
        \label{fig:augmented_scene} 
    \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/urdformer_nD_bigfont.pdf}
        \caption{The URDFormer architecture takes as input a cropped RGB image and object part boxes and predicts a hierarchy consisting of a base class and parent-child relations that make up the final URDF file. \todo{base category n=7, cabinet, oven, fridges, dishwasher, laundry washer, oven_fan, shelf}}
        \label{fig:urdformer} 
    \end{subfigure}
    \caption{URDFormer architecture and training procedure}
\end{figure*}

% \textbf{Scene Reconstruction} Constructing digital twins has gained popularity in robotics especially to bridge the gap between simulation and reality. Through robotic~\cite{nie2022structure, ma2023sim2real} or human~\cite{hsu2023ditto, jiang2022ditto} interaction data, the articulation and parts of the object are revealed and a simulated model can be reconstructed. Training policies on such a reconstructed scene can allow for zero-shot transfer.
% \method{} eliminates the need for prior interaction by leveraging large-scale pre-training and can reconstruct an unseen scene from a single RGB observation. We show that this scene is accurate enough to solve several real-world tasks in a zero-shot fashion.

\textbf{Data Augmentation with Generative Models}
Our work is certainly not the first ~\citep{syntheticsurvey} to use synthetic data generated by generative models for training networks that can then be deployed on real data. These models have been used the context of data augmentation ~\citep{chen23genaug, yu23rosie, trabucco23dataaug}, representation learning via self supervised learning ~\citep{fu23dreamsim, tian23stablerep, jahanian22genmodels}, model selection ~\citep{shoshan23synthetic} and even applications like healthcare ~\citep{choi17health}. In contrast to these works, our work shows that controllable generative modeling can be used to generate datasets that are suitable for inverse modeling for creating simulation assets at scale.  

% Others have used procedural generation [57, 31] and unsupervised learning [29] to synthesize grid-world
% environments for AI. TODO PROCTHOR description. TODO describe openrooms, HM3D. Openrooms - interactive but no articulation, very slow, requires more ground truth depth stuff. 

% Talk about how we don't just want to do procedureal generation, but instead we want to be controllable, and targeted to a particular image. Also we want things to be articulated and kinematically accurate. 

% \textbf{3-D reconstruction and Novel View Synthesis:}

% Discuss NeRF, splatting etc, zero123 and other techniques for 3-D reconstruction. Start with talking about methods for multi-view synthesis, then things for single view synthesis. But say how these don't really infer object level statistics, semantics and kinematics.  

% Then go to ditto in the house + follow ups. Say that they do but require ground truth depth + interaction. We do so from real-world RGB data without interaction etc. Old wolfram burgard paper too. Talk about how all of these need depth and interaction. We instead leverage semantics encoded in the generative mdoels. 




% Talk about how we use gen models for dataset generation. Talk about how this has been done for data augmentation - genaug, cacti, trabucco thing, etc. Also used for things like representation learning, classifier learning (isola and co). But then mention that in this work, we use the generative models for learning how to do inverse modeling from RGB to sim, not something that has been done before both in terms of solving inverse modeling problems or for the particular use case. 


% \subsection{Inverse Modeling as Supervised Learning}
% TODO: Describe the inverse modeling problem. 

% TODO: Describe how when you have a paired dataset, you can try and do inverse modeling this way. 

% \subsection{Simulation Representations}
% TODO: Describe URDF/USDZ and other forms of how simulation environments are represented. 

% \subsection{Controllable Generative Modeling}
% TODO: Describe how pre-trained generative models are able to take in controlled masks and generate realistic images piece by piece. 

==> tables/baseline_vision_backbone.tex <==
\begin{table}[hb]

\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{ccccc}
    
    \small \small Pre-training & \small $\text{ED Box}$ $\downarrow$ & \small $\text{ED IoU}_{0.25}$ $\downarrow$ & \small $\text{ED IoU}_{0.5}$ $\downarrow$ & \small $\text{ED IoU}_{0.75}$ $\downarrow$ \\
    \toprule
    None                        & 7.00                        & 6.15                              & 8.37                             & 14.48                             \\ 
    
    ImageNet         & 6.33                        & 5.48                              & 7.74                             & 13.85                             \\ 
    \midrule 
    
    MAE (RGB) & 6.19                        & 5.26                              & 7.63                             & 14.11                             \\ 
    
    MAE (bbox)                 & 7.04                        & 6.52                              & 8.26                             & 14.26                             \\ 
    \midrule 
    
    \textbf{MAE}   & \textbf{5.70}               & \textbf{5.11}                     & \textbf{7.07}                    & \textbf{13.41}                    \\
    \bottomrule
    
\end{tabular}
}
\caption{\footnotesize{\textbf{Ablation Study:} The results show training \method with different ViT backbones and input features. Training using both visual/spatial features, with a backbone pre-trained on diverse real images achieves higher performance.}}

\label{table:ablation_table}
% \vspace{-0.8cm}
\end{table}
